vlang: Mapping Verilog Netlists to Modern Technologies

Portability of hardware designs between Programmable Logic Devices (PLD) can be accomplished through the use of device-agnostic hardware description languages (HDL) such as Verilog or VHDL. Hardware designers can use HDLs to migrate hardware designs between devices and explore performance, area and power tradeoffs, as well as, port designs to an alternative device. However, if design files are corrupt or missing, the portability of the design is lost. While reverse engineering efforts may be able to recover an HDL-netlist of the original design, HDL-netlists use device-specific primitives, restricting portability. Additionally, the recovered design may benefit from other computational technologies (e.g., $\mu$P, GPGPUs), but is restricted to the domain of PLDs. In this work, we provide a new framework, vlang, which automatically maps Verilog-netlists into LLVM's intermediate representation (IR). The remapped design can use the LLVM-framework to target many device technologies such as: x86-64 assembly, RISC-V, ARM or to other PLDs with a modern high-level synthesis tool. Our framework is able to preserve the exact functionality of the original design within the software executable. The vlang-produced software executable can be used with other software programs, or to verify the functionality and correctness of the remapped design. We evaluate our work with a suite of hardware designs from OpenCores. We compare our framework against state-of-the-art simulators, thereby outlining our framework's ability to produce a fully-functional, cycle accurate software-executable. We also explore the usage of vlang as a front-end for high-level synthesis tools.

==> tikz/llvm_and_vlang.tex <==
\begin{figure}[tbh!]
    \centering
\begin{tikzpicture}[
  font=\rmfamily\footnotesize,
  every matrix/.style={ampersand replacement=\&,column sep=1cm,row sep=.6cm},
  source/.style={draw,thick,rounded corners,fill=yellow!20,inner sep=.3cm},
  process/.style={draw,thick,rounded corners,fill=blue!20, inner sep=.3cm},
  sink/.style={source,fill=green!20},
  datastore/.style={draw,very thick,shape=datastore,inner sep=.3cm},
  dots/.style={gray,scale=2},
  to/.style={->,>=stealth',shorten >=1pt,semithick,font=\rmfamily\scriptsize},
  every node/.style={align=center}]

  % Position the nodes using a matrix layout
  \matrix{
    \node[process] (a) {Verilog}; \& \& \node[source] (b) {Verilog};\\
     \node[source] (c) {\texttt{C/C++}}; \& \node[source] (d) {LLVM Optimizer}; \& \node[source] (e) {\texttt{ARM}};\\
     \node[source] (f) {\texttt{ruby}}; \& \& \node[source] (g) {\texttt{x86}};\\
  };

  % Draw the arrows between the nodes and label them.
  \draw[to,draw=blue!40] (a) to[bend right=20] (d);
  \draw[to] (c) -- (d);
  \draw[to] (f) to[bend left=20] node[midway,above] {} node[midway, left] {} (d);
  \draw[to] (d) to[bend right=20] node[midway, above, xshift=-0.2cm] {\normalsize HLS} (b);
  \draw[to, draw=blue!40] (a) to[bend right=20] node[midway, above, xshift=0.3cm] {\normalsize \texttt{vlang}} (d);
  \draw[to] (d) -- node[midway] {} (e);
  \draw[to] (d) to[bend left=20] node[midway] {} node[midway,left] {} (g);
  % Draw the dotted surrounding lines and add the labels as separate nodes
  % This is necessary because the anchor of the fitted node is always center

  \node[draw,dotted,fit=(a) (c) (f),inner sep=4ex,] (ACF) {};
  \node[above=-3ex of ACF] (ACFt) {Input Language};
  \node[draw,dotted,fit=(b) (e) (g),inner sep=4ex,] (BEG) {};
  \node[above=-3ex of BEG] (BEGt) {Output ISA};
\end{tikzpicture}    
    \caption{Overview of an LLVM-based HLS Compiler. }
    \label{fig:hls}
\end{figure}
